Partitioning Message Passing for Graph Fraud Detection

Label imbalance and homophily-heterophily mixture are the fundamental problems encountered when applying Graph Neural Networks (GNNs) to Graph Fraud Detection (GFD) tasks. Existing GNN-based GFD models are designed to augment graph structure to accommodate the inductive bias of GNNs towards homophily, by excluding heterophilic neighbors during message passing. In our work, we argue that the key to applying GNNs for GFD is not to exclude but to {\em distinguish} neighbors with different labels. Grounded in this perspective, we introduce Partitioning Message Passing (PMP), an intuitive yet effective message passing paradigm expressly crafted for GFD. Specifically, in the neighbor aggregation stage of PMP, neighbors with different classes are aggregated with distinct node-specific aggregation functions. By this means, the center node can adaptively adjust the information aggregated from its heterophilic and homophilic neighbors, thus avoiding the model gradient being dominated by benign nodes which occupy the majority of the population. We theoretically establish a connection between the spatial formulation of PMP and spectral analysis to characterize that PMP operates an adaptive node-specific spectral graph filter, which demonstrates the capability of PMP to handle heterophily-homophily mixed graphs. Extensive experimental results show that PMP can significantly boost the performance on GFD tasks.

==> 08_Related_Work.tex <==
\section{Related Work}


\textbf{Label Imbalanced Learning on Graphs.} GNNs are known to be sensitive to label imbalance~\citep{liu2023survey}. Currently, several studies have proposed different strategies to address this challenge, such as by implementing adversarial constraints \citep{shi2020multi}, generating minority instances using techniques like GAN \citep{qu2021imgagn} or SMOTE \citep{zhao2021graphsmote}, and modifying the degree of imbalance compensation \citep{song2022tam}.
% DR-GCN~\citep{shi2020multi} introduces conditional adversarial training to enhance the separation of nodes from different classes. TAM~\citep{song2022tam} address label imbalance by adaptively determining the intensity of imbalance compensation based on the local topology of individual nodes. 
% Other studies employ synthetic node generation techniques, particularly for minority classes, to tackle the label imbalance issue, such as utilizing GAN \citep{qu2021imgagn} or SMOTE \citep{zhao2021graphsmote}.
% ImGAGN~\citep{qu2021imgagn} is also an adversarial training framework, using a generator to produce fake minority nodes, simulating the distribution of real minority nodes, while a discriminator differentiates between real and generated nodes. Inspired by SMOTE~\citep{chawla2002smote}, GraphSMOTE~\citep{zhao2021graphsmote} constructs an intermediate embedding space using a feature extractor, employs interpolation to generate synthetic nodes, and simultaneously trains an edge generator and a GNN-based node classifier. 
Despite their effectiveness, their success heavily relies on augmenting graph structure to balance the label distribution, which can hardly be adaptive to fraud detection tasks on large-scale graphs. 
% \paragraph{Label Imbalanced Learning on Graphs.} GNNs are known to be sensitive to label imbalance~\citep{liu2023survey}. Currently, several studies have proposed different strategies to address this challenge. DR-GCN~\citep{shi2020multi} introduces a conditional adversarial training to enhance the separation of nodes from different classes. ImGAGN~\citep{qu2021imgagn} is also an adversarial training framework, using a generator to produce fake minority nodes, simulating the distribution of real minority nodes, while a discriminator differentiates between real and generated nodes. TAM~\citep{song2022tam} address label imbalance by adaptively determining the intensity of imbalance compensation based on the local topology of individual nodes. Inspired by SMOTE~\citep{chawla2002smote}, GraphSMOTE~\citep{zhao2021graphsmote} constructs an intermediate embedding space using a feature extractor, employs interpolation to generate synthetic nodes, and simultaneously trains an edge generator and a GNN-based node classifier. Despite their effectiveness, their success heavily relies on augmenting graph structure to balance the label distribution, which can hardly be adaptive to fraud detection tasks on large-scale graphs. 
% Graph imbalance learning methods can be broadly categorized into three groups: undersampling, oversampling, and cost-sensitive learning. Undersampling methods~\citep{yin2020novel, } reduce the number of majority class nodes or edges to make the graph more balanced. 
\textbf{Graph Heterophily Learning.} 
Heterophily has emerged as a significant concern for GNNs. This issue was initially highlighted by~\citet{DBLP:conf/iclr/PeiWCLY20}. Separating ego- and neighbor-embeddings~\citep{zhu2020beyond,platonov2023critical,hamilton2017inductive} proves to be an effective technique for learning on heterophilic graphs. Given that nodes sharing the same class are distantly placed within heterophilic graphs, several approaches aim to extend the local neighbors to non-local ones by integrating multiple layers~\citep{chien2021adaptive,abu2019mixhop}, and identifying potential neighbors through attention mechanisms~\citep{liu2021non,yang2022graph} or similarity measures~\citep{zhuo2022proximity,jin2021node}. Spectral-based methods~\citep{bo2021beyond,luan2021heterophily} overcome this challenge by introducing additional graph filters and mixture strategies. \textbf{GNN-based Fraud Detection.} 
GNNs have been leveraged to detect fraudulent activities in financial services~\citep{rao2021xfraud, xu2021towards,lin2021online}, telecommunications~\citep{nabeel2021cadue}, social networks~\citep{deng2022markov}, and healthcare~\citep{cui2020deterrent}. CARE-GNN~\citep{dou2020enhancing} employs a label-aware similarity measure to identify informative neighbors and leverages reinforcement learning to selectively integrate similar neighbors. PC-GNN~\citep{liu2021pick} utilizes label-balanced samplers for sub-graph training. Spectral-based methods~\citep{tang2022rethinking,gao2023ghrn} conduct spectral analysis on fraud graphs, designing band-pass or high-pass graph filters specifically tailored to detect fraud nodes. GAGA~\citep{wang2023label} groups neighbors by augmenting neighbor features with their labels explicitly and treat unlabeled neighbors as a new class. The basic idea of our PMP and GAGA is to use label information to enhance the message passing process. However, label-augmented features used in GAGA cannot resist the gradient bias caused by label imbalance. Besides, assigning pseudo-labels to unlabeled nodes potentially introduces noise in the model, especially if the pseudo-labels do not align well with the true underlying labels. 
